System 2 Reasoning Capabilities Are Nigh

In recent years, machine learning models have made strides towards human-like reasoning capabilities from several directions. In this work, we review the current state of the literature and describe the remaining steps to achieve a neural model which can perform System~2 reasoning analogous to a human. We argue that if current models are insufficient to be classed as performing reasoning, there remains very little additional progress needed to attain that goal.

==> preamble_arxiv.tex <==
\usepackage{geometry}

\geometry{
    textheight=22cm,
    textwidth=16cm,
    top=3cm,
    headheight=12pt,
    headsep=25pt,
    footskip=30pt,
}

\usepackage{lmodern}
\usepackage{natbib}
